Dynamic View Synthesis from Dynamic Monocular Video

We present an algorithm for generating novel views at arbitrary viewpoints and any input time step given a monocular video of a dynamic scene. Our work builds upon recent advances in neural implicit representation and uses continuous and differentiable functions for modeling the time-varying structure and the appearance of the scene. We jointly train a time-invariant static NeRF and a time-varying dynamic NeRF, and learn how to blend the results in an unsupervised manner. However, learning this implicit function from a single video is highly ill-posed (with infinitely many solutions that match the input video). To resolve the ambiguity, we introduce regularization losses to encourage a more physically plausible solution. We show extensive quantitative and qualitative results of dynamic view synthesis from casually captured videos.

==> figure/fig_ablation_flow_reg.tex <==
\begin{figure}[t]
%
\newlength\figwidthflowreg
\setlength\figwidthflowreg{0.495\linewidth}
% 
\parbox[t]{\figwidthflowreg}{\centering%
  \fbox{\includegraphics[trim=270 60 40 45, clip=true, width=\figwidthflowreg]{fig/Ablation/Flow_reg/Skating_v000_t009_ablation_noflow_reg_img.png}}\\
  \small \emph{Without} motion regularization}%
%
\hfill
%
\parbox[t]{\figwidthflowreg}{\centering%
  \fbox{\includegraphics[trim=270 60 40 45, clip=true, width=\figwidthflowreg]{fig/Ablation/Flow_reg/Skating_v000_t009_ablation_flow_reg_img.png}}\\
  \small \emph{With} motion regularization}%
% left, bottom, right and top
\vspace{\figcapmargin}
\caption{\textbf{Motion regularization.} Regularizing our scene flow prediction in dynamic NeRF can help handle videos with large object motion. 
}
\label{fig:ablation_flow_reg}
\end{figure}

==> figure/fig_ablation_full.tex <==
\begin{figure}[t]
%
\newlength\figwidthfull
\setlength\figwidthfull{0.317\linewidth}
% 
\mpage{0.01}{\rotatebox[origin=c]{90}{\small  \quad With \quad \quad Without \quad}}
\parbox[t]{\figwidthfull}{\centering%
  \fbox{\includegraphics[trim=100 40 100 80, clip=true, width=\figwidthfull]{fig/Ablation/Full/Truck_v000_t003_ablation_nofull_img_d.png}}\\
  \fbox{\includegraphics[trim=100 40 100 80, clip=true, width=\figwidthfull]{fig/Ablation/Full/Truck_v000_t003_ablation_full_img_d.png}}\\
	\small Dynamic}%
%
\hfill
%
\parbox[t]{\figwidthfull}{\centering%
  \fbox{\includegraphics[trim=100 40 100 80, clip=true, width=\figwidthfull]{fig/Ablation/Full/Truck_v000_t003_ablation_nofull_img_s.png}}\\
  \fbox{\includegraphics[trim=100 40 100 80, clip=true, width=\figwidthfull]{fig/Ablation/Full/Truck_v000_t003_ablation_full_img_s.png}}\\
	\small Static}%
%
\hfill
%
\parbox[t]{\figwidthfull}{\centering%
  \fbox{\includegraphics[trim=100 40 100 80, clip=true, width=\figwidthfull]{fig/Ablation/Full/Truck_v000_t003_ablation_nofull_img.png}}\\
  \fbox{\includegraphics[trim=100 40 100 80, clip=true, width=\figwidthfull]{fig/Ablation/Full/Truck_v000_t003_ablation_full_img.png}}\\
	\small Composite}%
% left, bottom, right and top
\vspace{\figcapmargin}
\caption{\textbf{Full rendering loss.} Adding supervision on the composite model leads to improved novel view rendering.
}
\label{fig:ablation_full}
\end{figure}

==> figure/fig_consistency.tex <==
\begin{figure}[t!]
\begin{overpic}[width=1\linewidth]{fig/Consistency_v2.pdf}
% \begin{overpic}[width=1\linewidth,grid,tics=5]{fig/Consistency_v2.pdf}
\put (53, 37) {$\sfw(\r, t)$}
\put (6, 48) {$\sfw(\r + \sbw(\r, t), t - 1)$}
\put (55, 50) {$\sbw(\r + \sfw(\r, t), t + 1)$}
\put (29, 34) {$\sbw(\r, t)$}
% \put (16, 40) {$\mathcal{L}$}
% 
\put (15, 4) {$t - 1$}
\put (43, 4) {$t$}
\put (82, 12) {$t + 1$}
\end{overpic}
\vspace{\figcapmargin}
\caption{\textbf{Scene flow cycle consistency loss.}
To regularize the consistency of the scene flow, we have the scene flow cycle consistency regularization on $\sfw$ and $\sbw$.
}
\label{fig:consistency}
\end{figure}

==> overview.tex <==
\section{Overview}
\label{sec:overview}

% Introduce your problem with a toy example

% This figure illustrate the overall process of the algorithm, starting from inputs, processing steps, and outputs. Use forward references the figures with the corresponding equations and sections in the paper.
\input{figure/fig_overview}
